SureFED: Robust Federated Learning via Uncertainty-Aware Inward and Outward Inspection

In this work, we introduce SureFED, a novel framework for byzantine robust federated learning. Unlike many existing defense methods that rely on statistically robust quantities, making them vulnerable to stealthy and colluding attacks, SureFED establishes trust using the local information of benign clients. SureFED utilizes an uncertainty aware model evaluation and introspection to safeguard against poisoning attacks. In particular, each client independently trains a clean local model exclusively using its local dataset, acting as the reference point for evaluating model updates. SureFED leverages Bayesian models that provide model uncertainties and play a crucial role in the model evaluation process. Our framework exhibits robustness even when the majority of clients are compromised, remains agnostic to the number of malicious clients, and is well-suited for non-IID settings. We theoretically prove the robustness of our algorithm against data and model poisoning attacks in a decentralized linear regression setting. Proof-of Concept evaluations on benchmark image classification data demonstrate the superiority of SureFED over the state of the art defense methods under various colluding and non-colluding data and model poisoning attacks.

==> 8_Conclusion.tex <==
\section{Conclusion}
In this work, we provided theoretical and experimental analysis for our proposed federated learning algorithm, \sys{}, to show its robustness against data and model poisoning attacks. In particular, we experimentally showed the performance of \sys{} in Label-Flipping and Trojan data poisoning attack, in addition to Bit-Flip, A Little is Enough, and General Random model poisoning attacks. Furthermore,  we theoretically showed that  \sys{} is robust against Label-Flipping data poisoning attack and General Random model poisoning attack in a linear regression problem. One of the important features of our algorithm is that  its robustness against data/ model poisoning attacks does not require the majority of benign nodes over the compromised ones and holds against a wide range of poisoning attacks. 
